Multiresolution Transformer Networks: Recurrence is Not Essential for Modeling Hierarchical Structure

The architecture of Transformer is based entirely on self-attention, and has been shown to outperform models that employ recurrence on sequence transduction tasks such as machine translation. The superior performance of Transformer has been attributed to propagating signals over shorter distances, between positions in the input and the output, compared to the recurrent architectures. We establish connections between the dynamics in Transformer and recurrent networks to argue that several factors including gradient flow along an ensemble of multiple weakly dependent paths play a paramount role in the success of Transformer. We then leverage the dynamics to introduce {\em Multiresolution Transformer Networks} as the first architecture that exploits hierarchical structure in data via self-attention. Our models significantly outperform state-of-the-art recurrent and hierarchical recurrent models on two real-world datasets for query suggestion, namely, \aol and \amazon. In particular, on AOL data, our model registers at least 20\% improvement on each precision score, and over 25\% improvement on the BLEU score with respect to the best performing recurrent model. We thus provide strong evidence that recurrence is not essential for modeling hierarchical structure.

==> transformer.tex <==
\section{Encoder}
\noindent We first focus on the encoder. For each layer $\ell \in [L]$, let $W_{\ell, 1} \in \mathbb{R}^{d \times d_f}, b_{\ell, 1} \in \mathbb{R}^{1 \times d_f}, W_{\ell, 2} \in \mathbb{R}^{d_f \times d}$, and  $b_{\ell, 2} \in \mathbb{R}^{1 \times d}$ be the parameters to be learned such that $d_f > d$.   Let $E_{\ell} \in \mathbb{R}^{n \times d}$ be the output of layer $\ell$ of the encoder $E$, and let $\hat{E}_{\ell}$ be an intermediate result at layer $\ell$. Let $\sigma(X)$ denote the probabilities obtained by applying softmax on each row of $X$ independently, and likewise let $\psi(X)$ denote the layer normalization of each row of $X$, and let $\phi(X)$ be the result of applying the ReLU activation on $X$ elementwise. Let $\mathbb{I}_{n}$ denote the $n \times n$ identity matrix, and $1_n\in \mathbb{R}^n$ denote an $n$-dimensional column vector of all ones.  We have the following equations for the single head encoder $E$ that takes the source matrix $X_s$ as the input. \\ 

\noindent {\bf Single-attention encoder}
\begin{eqnarray*}
E_{0} & = & \sqrt{d} X_s   \\
\hat{E}_{\ell} & = & \left(\mathbb{I}_n + \sigma\left(\dfrac{E_{\ell-1} E_{\ell-1}^{\top}}{\sqrt{d}}\right) \right)E_{\ell-1}, \quad \ell \in [L] \\
E_{\ell} & = &  \psi \left( \psi(\hat{E}_{\ell}) +  \phi\left(\psi(\hat{E}_{\ell}) W_{\ell, 1} + 1_{n} b_{\ell, 1} \right) W_{\ell, 2} + 1_n b_{\ell, 2} \right), ~~~ \ell \in [L]. \\
\end{eqnarray*}

\noindent We take a closer look at these encoder equations. We write these equations in a more familiar form that is reminiscent of the RNNs. 

\begin{eqnarray*}
X_{\ell} & = & \psi(\hat{E}_{\ell})\\
H_{\ell} & = & \phi(X_{\ell} W_{\ell, 1}  + 1_{n} b_{\ell, 1} )\\ 
E_{\ell} & = &  \psi \left(X_{\ell} + H_{\ell} W_{\ell, 2} + 1_n b_{\ell, 2} \right), \qquad \ell \in [L]. \\
Y_{\ell} & = & E_{\ell}.
\end{eqnarray*}

\noindent Compare this notation with the simple RNN (Elman network) which takes the following form ($\beta_h$ and $\beta_y$ are activation functions):
\begin{eqnarray*}
h_{t} & = & \beta_h(W_h x_t + U_h h_{t-1} + b_h) \\
y_t & = & \beta_y(W_y h_t + b_y) \\
\end{eqnarray*}
Clearly, $H_{\ell}$ and $Y_{\ell}$ look very similar to $h_t$ and $y_t$ but for two differences. There is no counterpart of $U_t$ in $H_{\ell}$ since $H_{\ell}$ already contains representations at the sentence level (unlike RNN where the hidden representations are generated in sequence). Additionally, there is no $x_t$ in $y_t$ due to lack of the residual connection. 

\section{Decoder}
\noindent We now describe the decoder $D$. Note that unlike encoder, where the attention is bi-directional, the decoder should not attend to the words that have not been decoded yet. We will assume a mask $M_k$ that prevents information (attention) flow from words that have yet not been decoded by time $k$. $M_k$ is a matrix with entries 1 corresponding to valid coordinates and $- \infty$ otherwise. We will denote the elementwise matrix multiplication (Hadamard product) by $\odot$.  The decoder also consists of $L$ levels, and we denote the output from layer $\ell \in [L]$ at time $k \in [m]$ by $D_{\ell, k}$.  We also denote the intermediate results at any layer $\ell \in [L]$ by $\hat{D}_{\ell, k}$ and $\tilde{D}_{\ell, k}$.  We denote the decoder parameters by underlines, e.g., $\underline{W}_{\ell, 1}$. We denote the output probabilities for position $k$ by $O_k$.  The decoder acts on the target matrix $X_t$ and we have the following equations.\\

\noindent {\bf Single-attention decoder}
\begin{eqnarray*}
D_{0, k} & = & \sqrt{d} X_t,  \qquad  k  \in [m] \\
\hat{D}_{\ell, k} & = & D_{\ell-1, k} + \sigma\left(M_k \odot \dfrac{D_{\ell-1, k} D_{\ell-1, k}^{\top}}{\sqrt{d}}\right) D_{\ell-1, k}, \hspace{3cm} \ell \in [L], k \in [m] \\
\tilde{D}_{\ell, k} & = &\psi(\hat{D}_{\ell, k}) + \sigma\left(\dfrac{\psi(\hat{D}_{\ell, k}) E_{L}^{\top}}{\sqrt{d}}\right) E_{L}, \hspace{4.5cm} \ell \in [L], k \in [m] \\
D_{\ell, k} & = &  \psi\left(\psi(\tilde{D}_{\ell, k}) +  \phi\left(\psi(\tilde{D}_{\ell, k}) \underline{W}_{\ell, 1} + 1_{n} \underline{b}_{\ell, 1} \right) \underline{W}_{\ell, 2} + 1_n \underline{b}_{\ell, 2}\right), \hspace{1cm} \ell \in [L], k \in [m] \\
O_k & = &  k^{th} \text{ column of } \sigma(D_{L, k} B_{emb}), \\
\end{eqnarray*}

\color{red} TODO: write $O_k$ formally using matrix operations that  filter out $k^{th}$ column. Also check if it is $k^{th}$ column or row.  \color{black} 

\noindent where $B_{emb}$ is the same matrix that was used for generating the source and target embeddings. 

\section{Multi-attention}
\noindent The idea of multi-attention is to transform the inputs, to each attention layer, via $P$ learned linear projections, perform a separate attention on the result of each projection in parallel, concatenate these attentions, and then do a final linear tranformation (which acts like an inverse projection).   A multi-attention encoder takes the following form, where $Z_{\ell, i}^1$, $Z_{\ell, i}^2$, $Z_{\ell, i}^3 \in \mathbb{R}^{d \times d_p},  Z_{\ell, i}^4 \in \mathbb{R}^{d_p \times d},  \ell \in [L], i \in [P]$ are additional parameters to be learned, and $d_p = d/P$. We below provide a weighted attention \cite{AKS2017} based decoder that learns to weight the different attentions, unlike \cite{V2017} who treat all the attentions equally.   \cite{AKS2017} enforced $\sum_i \alpha_{\ell, i} = \sum_i \kappa_{\ell, i} = 1$, and $\alpha_{\ell, i}, \kappa_{\ell, i} > 0$ for all $\ell \in [L], i \in [P]$ to obtain a distribution over the attentions. The weighted attention showed improved performance at the expense of few additional learned parameters, i.e., $\kappa_{\ell, i}, \alpha_{\ell, i}, i \in [P]$   \cite{AKS2017}.\\

\clearpage
\noindent {\bf Multi-attention encoder}
\begin{eqnarray*}
E_{0} & = & \sqrt{d} X_s  \\
\hat{E}_{\ell, i} & = & \kappa_{\ell, i} \left(\mathbb{I}_n + \sigma\left(\dfrac{E_{\ell-1} Z_{\ell, i}^1 Z_{\ell, i}^{2^{\top}} E_{\ell-1}^{\top}}{\sqrt{d}}\right) \right)E_{\ell-1} Z_{\ell, i}^3 Z_{\ell, i}^4, \qquad \ell \in [L], i \in [P]  \\
\hat{E}_{\ell} & = &  \sum_{i \in [P]} \alpha_{\ell, i}  \hat{E}_{\ell, i}, \qquad \ell \in [L]\\
E_{\ell} & = &  \psi \left( \psi(\hat{E}_{\ell}) +  \phi\left(\psi(\hat{E}_{\ell}) W_{\ell, 1} + 1_{n} b_{\ell, 1} \right) W_{\ell, 2} + 1_n b_{\ell, 2} \right), \qquad \ell \in [L]. \\
\end{eqnarray*}

\noindent The same idea could be applied to build multi-attention in the decoder as well, and we omit the details.


